On Dynamic Mode Decomposition of Control-affine Systems

This paper builds on the theoretical foundations for dynamic mode decomposition (DMD) of control-affine dynamical systems by leveraging the theory of vector-valued reproducing kernel Hilbert spaces (RKHSs). Specifically, control Liouville operators and control occupation kernels are used to separate the drift dynamics from the input dynamics. A provably convergent finite-rank estimation of a compact control Liouville operator is obtained, provided sufficiently rich data are available. A matrix representation of the finite-rank operator is used to construct a data-driven representation of its singular values, left singular functions, and right singular functions. The singular value decomposition is used to generate a data-driven model of the control-affine nonlinear system. The developed method generates a model that can be used to predict the trajectories of the system in response to any admissible control input. Numerical experiments are included to demonstrate the efficacy of the developed technique.

==> Reviews.tex <==
\clearpage
\onecolumn\setcounter{page}{1}%\setstretch{1.8}

\begin{center}
    \large\textbf{Response to Review Comments}
\end{center}


\begin{center}
    \textbf{Response to the comments by the associate editor}
\end{center}
Your paper has been evaluated by 4 reviewers. Here is a
list of main pros and cons shared by the reviewers.
Pros
\begin{enumerate}


\item The paper introduces a unique approach using Dynamic
Mode Decomposition (DMD) for identifying control-affine
systems, with convergence proofs for finite-rank
approximations.
\item The Duffing oscillator example effectively demonstrates
the method in a nonlinear system.
\item Reviewers appreciate the high-level math, especially for
those familiar with Koopman theory, RKHS, and Liouville
operators.
\item The paper is valuable for nonlinear system
identification and control-affine applications.


\end{enumerate}
Cons
\begin{enumerate}
\item  Reviewers find the paper overly dense and hard to
follow, suggesting it could be more accessible for a
broader audience.
\item Comparison with other methods like SINDy and SSM is
lacking, which would help position the approach.
\item Reviewers find certain aspects unclear, such as kernel
choice, parameters, and finite-rank approximations.
\item Varied parameter \( M \) values would strengthen the
convergence analysis.
\item More clarity on dynamical system assumptions is needed.
\item Reviewers note heavy self-citation and suggest including
recent relevant literature.
\item Reviewers noted some typos and undefined acronyms.



\end{enumerate}
Conclusion
In summary, the paper is seen as a valuable contribution
with rigorous theory and practical applications. Enhancing
readability, adding comparisons, clarifying details, and
broadening references will improve its appeal and impact.



\clearpage
\onecolumn
\begin{center}
    \textbf{Response to the comments by Reviewer 1 (1461)}
\end{center}
This paper presents a novel approach based on the
principles of Dynamic Mode Decomposition (DMD) for
identifying control-affine dynamical systems.

The majority of the paper is focused on developing the
proposed method, culminating in the SCLDMD algorithm. By
the way, I noticed that the acronym "SCLDMD" is never
explicitly defined in the text. Additionally, the authors
provide convergence proofs for the finite-rank estimation
of a compact control Liouville operator.

Overall, the paper is well-structured, reasonably
accessible, and appears to be a valuable contribution to
the field of nonlinear system identification. Given my
limited expertise in Reproducing Kernel Hilbert Spaces
(RKHSs) and control Liouville operators, my comments and
questions primarily pertain to the Numerical Experiments
section:
\begin{enumerate}


\item How does the choice of kernel and associated parameters
impact the accuracy of the system identification?
\\ {\color{red} I think it is clear that we don't have error bounds in this paper, and we can't predict the accuracy of the system identification using any finite data set using any kernel or parameter.}
\item Could you elaborate on the specific parameter choices for
the Duffing oscillator? Specifically, what was the
rationale for considering only the undamped dynamics in
this case?
\\ {\color{red} The undamped system is not asymptotically stable. Should we add a comment about this?}
\item A potentially related question: is the proposed method
suitable for systems that exhibit sensitivity to initial
conditions?
\\ {\color{red} In figure 2, we see the error increasing over time for this system. If the system is highly sensitive to the initial conditions, then the prediction will be large. Should we add a comment about this?}
\item In figure 2, it seems that the error for x2 is increasing
with time (and possibly also for x1, though to a lesser
extent). Could you provide an explanation for this trend?
\\ {\color{red} The approximation is not exact.}
\item In Figure 3, it seems that error norms are displayed, but
the type of norm used is not specified. Would it be
feasible to plot the error for each vector component
separately (or compare the true and estimated components
directly, without computing the error)? This could help
better assess the method's ability to approximate the true
drift dynamics and control effectiveness functions.
{\color{red} Corrected the norm is shown as the vector norm. If we plot the true and estimated components
directly, without computing the error, i don't think we can deduce anything. }
\item Finally, I believe the relevance of this method would be
enhanced if compared to established approaches such as for
example SINDYc (already cited in the manuscript), Operator
Inference (from K. Willcox's group) and Spectral
SubManifold (SSM, from G. Haller's group).
{\color{red} Comparisons ar planned for the journal paper}




\end{enumerate}

\clearpage
\onecolumn
\begin{center}
    \textbf{Response to the comments by Reviewer 2 (3049)}
\end{center}
Similar material appears in recent TAC and SIAM papers, so
this paper may be valuable to an audience wanting to
understand the ideas and methods. Although the level of
math is impressive, the writing is dense and hard to
follow. The authors may wish to consider writing papers
that are more accessible to readers. 

The numerical example seems to require a large amount of
data.  A comparison to SINDy or other methods might be
useful for readers.  
\\
{\color{red}Comparisons are planed for the journal paper.}


\clearpage
\onecolumn
\begin{center}
    \textbf{Response to the comments by Reviewer 3 (6743)}
\end{center}
The paper introduces a kernel-based approximation technique
for Koopman operators of control affine systems. Most
importantly, the authors prove that their approach yields
convergence of finite-rank-approximations. The approach is
verified using the popular Duffing example in the numerics
section.

While I am generally positive about the paper, I have two
major concerns. 
\begin{enumerate}


\item I find the statements in Section IV somewhat irritating.
If the story of the paper is to promote finite-rank
approximations, then the limit "$M \to \infty$" is not very
helpful, in my opinion. So what is the use of a finite-rank
analysis, if the theorem only holds in the limit? That
being said, using M=225 in the example is far from $\infty$,
obviously. So the example does not support the study of
convergence at all. The authors should at least consider
several different values for M in the numerics.
\\{\color{red} should we add an experiment with M=50?}
\item The list of references is somewhat limited, and a large
number of references is to the authors' own work, partially
in preprint form. I suggest to add a more thorough
literature overview. For instance, there are many works on
RKHS approximations of Koopman operators, e.g.,


\begin{enumerate}
\item https://doi.org/10.1007/s00332-019-09574-z
\item https://doi.org/10.1016/j.acha.2024.101657
\item https://doi.org/10.1016/j.acha.2017.09.001
\item https://doi.org/10.1088/1361-6544/ad4ade
\end{enumerate}
In the same manner, there are also many works on bilinear

Koopman models, such as
\begin{enumerate}
\item https://doi.org/10.1137/20M1325678
\item https://doi.org/10.1109/LRA.2021.3068117
\item https://doi.org/10.1007/s00332-022-09862-1
\end{enumerate}
\end{enumerate}

\clearpage
\onecolumn
\begin{center}
    \textbf{Response to the comments by Reviewer 4 (10761)}
\end{center}
The paper proposes a learning procedure of control-affine dynamical systems based on Liouville
operator and RKHS. The novelty of the paper is well explained in the introduction, showing that on the
one hand Liouville operator and RKHSs have been explored in the literature, but without control, and
on the other hand, extended DMD for control dynamical systems exists, but no convergence guaranties
are provided. The present paper fills this gap. It can be viewed as a follow-up of Abudia et al. (IFAC
2024). Theoretical statement of the problem is presented at the continuous level, then finite-rank and
matrix representations are defined and convergence results are provided. The study ends with the
proposition of an algorithm and with a numerical test on non-linear oscillator.
I find the paper well conducted and provides some novelty. Some specific aspects remain unclear
to me, and I believe that some clarifications are required before I can recommend it for publication.

\begin{center}
    \textbf{General comments}
\end{center}
\begin{enumerate}

   \item  In the introduction, the approach of Strässer et al. (2024) has been criticised pointing the difficulty
of learning an unstable system in open loop. It is not clear to me if (and how) this issue is solved
with the proposed method.
\\{\color{red} The theory doesn't require a system to be stable, and the simulation uses an undamped duffing oscillator, which is not stable.}

\item A connected question, probably out of the scope of the paper, but important for control application
is: how efficient is the learning of the open-loop system for closed-loop applications? How
the proposed method is positioned compared to other methods?
\\{\color{red} not sure what he means by efficient. }

\item In the formalism, phase-space (through RKHS) integrations are performed by time integrations. This suggests a sort of ergodicity assumption. What are the hypotheses on the dynamical system?
\\{\color{red} It is clearly stated that we are only considering control-affine systems. we don't assume ergodicity.}
\item Proposition 2 is not formulated clearly enough to me regarding what is chosen and what is deduced. Is $\Gamma_{\theta, u}^{(s)}$ of the form stated equation (1)? Or what is the link between $K_{\theta(t)}$ and $\Gamma$ ? The kernel is chosen, which sets $\Gamma_{\theta, u}^{(s)}$ ? Please clarify.
\\{\color{red} (1) is inside Proposition 2}.
\item In Definition 2: $\tilde{H}_d$ space is not clearly defined. Same question for $d$.
\\{\color{red} added the clarification "where $\tilde{H}_{d}$ is a scaler valued RKHS."}
\item How the method scales with the dimension of the dynamical system $n$ ? Could it be related to the error bound Lemma 1 associated with the RKHS norm?
\\{\color{red} The method works for any $n$. Is asking about computation complicity with respect to $n$?}
\item In proof of proposition $6, A_{f, g}^* \beta_j=d_j$ suggests that $A_{f, g}^*=A_{f, g}^{-1}$, and then that the control Liouville operator is skew symmetric. Is it trivial or a remark should be added? Is it restricted to invertible dynamics?
\\{\color{red} Not sure what he means}.
\item Possibly variable time integration $T$ are mentioned to provide density arguments. In SCLDMD, $T$ is fixed. Is it possible to learn a set of trajectories of different times? If not, is there some theoretical restrictions based on possibly unachieved density assumptions?
\\{\color{red} We use different times such as $T_i$ which can be different for each trajectory $u_i$}
\item Convergence is a major contribution of the present work. In the results section, quantifying the estimation error with respect to $M$ (averaged over a set of test controls/initial conditions) is expected. One may ask ourselves how fast is the convergence.
\\{\color{red} We don't have an error bound in this paper.}

    
\end{enumerate}

\begin{center}
    \textbf{Minor comments and typos}
\end{center}

\begin{enumerate}
\item “using compact a control Liouville operator.” $\mapsto$ to reformulate “a compact”?
\\ {\color{red} Corrected.}

\item Just before Proposition 4 : “int he” $\mapsto$ “in the”
\\ {\color{red} Corrected.}

\item Around equation (12) the sentence ends prematurely.
\\ {\color{red} Corrected.}

\item In Algogorithm 1, line 5: the second left arrow should be removed.
\\ {\color{red} Corrected.}
\end{enumerate}


